Zeroth-order Deterministic Policy Gradient

Deterministic Policy Gradient (DPG) removes a level of randomness from standard randomized-action Policy Gradient (PG), and demonstrates substantial empirical success for tackling complex dynamic problems involving Markov decision processes. At the same time, though, DPG loses its ability to learn in a model-free (i.e., actor-only) fashion, frequently necessitating the use of critics in order to obtain consistent estimates of the associated policy-reward gradient. In this work, we introduce Zeroth-order Deterministic Policy Gradient (ZDPG), which approximates policy-reward gradients via two-point stochastic evaluations of the $Q$-function, constructed by properly designed low-dimensional action-space perturbations. Exploiting the idea of random horizon rollouts for obtaining unbiased estimates of the $Q$-function, ZDPG lifts the dependence on critics and restores true model-free policy learning, while enjoying built-in and provable algorithmic stability. Additionally, we present new finite sample complexity bounds for ZDPG, which improve upon existing results by up to two orders of magnitude. Our findings are supported by several numerical experiments, which showcase the effectiveness of ZDPG in a practical setting, and its advantages over both PG and Baseline PG.

==> problem1.tex <==
%!TEX root = root1.tex
% Think of a diffrent title, but in this section, we are going to derive the overall framework in which RL is a specific example.
\section{Assumptions}

These are the assumptions I need to formalize and add.
\begin{assumption} \label{asm:DCT_cond}
	Conditions required for DCT to hold, namely $\mathcal{X}$ is bounded and compact and $f$ and $\phi$ are bounded by constants.
\end{assumption}

\begin{assumption}\label{asm:bounded_gradient}
	The gradient of the policy is bounded by some constant $C_1$
\end{assumption}


\begin{assumption} \label{asm:bounded_Q}
	The $Q$ function cannot be larger than $\mathcal{Q}$
\end{assumption}

\begin{assumption}
	The objective function is $L$-smooth and $G$-Lipschitz. The smoothed objective is therefore also $L$-smooth and $G$-Lipschitz. (I think there is a lemma which relates this)
\end{assumption}


\section{Zeroth Order Stochastic Compositional Gradient Descent}
Let $\mathcal{X}$ and $\mathcal{Y}$ be closed and compact subsets of $\mathbb{R}^n$ and $\mathbb{R}^m$ respectively. We consider the optimization problem 
%
\begin{equation} \label{equ:main_problem}
\min_{x\in \mathcal{X}} F(x) := (f \circ g)(x),
\end{equation}
%
where $g:\mathcal{X} \to \mathcal{Y}$ is deterministic and $f: \mathcal{Y} \to \mathbb{R}$ is random in $v$ by 
%
\begin{equation}
f(y) = \mathbb{E} \left[f_v(y)\right].
\end{equation}
% 
In particular, we consider the case where only zeroth order information on $f$ can be obtained by some oracle. This is a major distinction from \cite{wang2017stochastic} which considers the case minimizing nested expectations with first order information on the outer function. \cite{wang2017stochastic} mentioned in their analysis that zeroth order methods to solve the problem were possible, but did not derive algorithms or convergence rates for this case.

This work looks to derive a zeroth order algorithm to solve (\ref{equ:main_problem}) and characterize its convergence rate. Deterministic policy gradient \cite{silver2014deterministic} and \emph{ANOTHER PROBLEM} are examples of types of problems which fit this framework. In fact, \cite{vemula2019contrasting} derives the convergence rate for deterministic policy gradient with a finite horizon action space exploration. Our convergence analysis fits the broader class of non-Markovian transition distributions and the infinite horizon case. Our derived rate is a strict improvement of existing rates. 

To apply SGD, we need an unbiased sample of $\nabla F$ at a given $x$, which by chain rule becomes
%
\begin{equation}
\nabla F(x) = \nabla g(x) \nabla f(g(x)) = \nabla g(x) \nabla \mathbb{E} \left[f_v(g(x))\right]
\end{equation}
%
Because $g(x)$ is known and differentiable, $\nabla g(x)$ is known explicitly. As such, the challenge lies in finding an estimate of $\nabla \mathbb{E}\left[f_v(g(x))\right]$ using only zeroth order information on $f_v$. By Assumption \ref{asm:DCT_cond}, we can bring the gradient inside the expectation, and so we are tasked to find a means to estimate $\nabla f_v(g(x))$ using only zeroth order samples of $f_v$.

By introducing Gaussian smoothing, derivative free estimates of the gradient can be obtained by only using zeroth order information \cite{nesterov2017random}. Let $\mu > 0$ be a smoothing parameter and define the smoothed function $\tilde f_v : \mathcal{Y} \to \mathbb{R}$ to be 
%
\begin{equation}
\tilde f_v^\mu (y) = \mathbb{E}_{u \sim \mathcal{N}(0,I_m)} \left[ f_v(y + \mu u) \right].
\end{equation}
% 
With slight abuse of notation, we let $\tilde f$ be shorthand notation for $\tilde f_v^\mu$. For $u \sim \mathcal{N}(0,I_m)$, evaluating
%
$$\frac{f_v(y+\mu u) - f_v(y)}{\mu} u$$
%
is known to be an unbiased estimate of the smoothed function $\tilde f$ which is related by the smoothing parameter $\mu$ to the true gradient of the original function $f_v$ \cite{nesterov2017random}. 

Using this insight, we propose the Algorithm \ref{alg:ZO_SCGD} to solve problem (\ref{equ:main_problem}).

\begin{algorithm}
	\label{alg:ZO_SCGD}
	\caption{Zeroth Order SCGD}
	\begin{algorithmic}
		\REQUIRE $x_0$, $\mu, \eta$
		\FOR{$t = 0, 1, \dots$}
		\STATE Explicitly evaluate $\Psi_t \leftarrow \nabla_x g(x_t)$
		\STATE Sample $u \sim \mathcal{N}(0,I_m)$
		\STATE Query oracle $f^+ \leftarrow f_v(g(x) + \mu u)$
		\STATE Query oracle $f^- \leftarrow f_v(g(x))$
		\STATE $h_{t}\leftarrow  \Psi_t \frac{f^+ - f^-}{\mu}u$ 
		\STATE $x_{t+1} \leftarrow x_t + \eta h_t$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\section{Convergence rate of Algorithm \ref{alg:ZO_SCGD}}
In this section, we derive the convergence rate of Algorithm \ref{alg:ZO_SCGD}. To do so, we need to establish that the expected value of $g_t$ is an unbiased estimate of the gradient of the smooth function and that $g_t$ has bounded variance. These are established in the following two lemmas.

\begin{lemma}
	$h_t$ is an unbiased estimate of $\nabla \tilde f$
\end{lemma}
\begin{proof}
	By \cite{nesterov2017random}, we know that $\mathbb{E}\left[\frac{f_v(g(x) + \mu u) - f_v(g(x))}{\mu}u\right]$ is an unbiased estimate of $\nabla \tilde f$. The rest follows by construction.
\end{proof}

\begin{lemma}
	$\mathbb{E}[\|h_t - \mathbb{E}[h_t] \|_2^2] < \infty$
\end{lemma}

\begin{proof}
	Because the estimate is unbiased, all we need to show is that $\mathbb{E}\left[\|h_t\|^2_2\right] < \infty$. By Algorithm \ref{alg:ZO_SCGD}, we have 
	\begin{equation}
	\E[\|h_t\|^2] = \E[\|\nabla_x g(x) \frac{f^+ - f^-}{\mu}u \|^2]
	\end{equation}
	By Cauchy-Schwartz, we have
	\begin{equation}
	\E[\|h_t\|^2] \leq \E[\|\nabla_x g(x)\|^2\| \frac{f^+ - f^-}{\mu}\|^2\|u \|^2]
	\end{equation}
	We bound $\nabla g(x)$ by Assumption \ref{asm:bounded_gradient} and the difference $f^+-f^-$ by Assumption \ref{asm:bounded_Q}. As such, we arrive at the bound
	\begin{equation}
	\E[\|h_t\|^2] \leq \frac{4C_1^2Q^2}{\mu^2} \E [\|u \|^2] =  \frac{4mC_1^2Q^2}{\mu^2}=:V
	\end{equation}
	
\end{proof}

Now that we have established that the estimate $h_t$ is unbiased and has bounded variance, we can apply the stochastic gradient descent convergence rate for the smoothed function $\tilde f$ as is done by \cite{vemula2019contrasting} using the analysis of \cite{ghadimi2013stochastic}.

\begin{theorem} With $\tilde f$ L-smooth and G-Lipshitz, then
	$$\sum_{t = 1}^T \E\left[\|\nabla x \tilde f \|^2\right]\leq \frac{1}{\eta} \Delta_0 + LT\eta (V + G^2) $$
	Further, if $\eta = T^{-1/2}$, then
	$$\frac{1}{T}\sum_{t = 1}^T \E\left[\|\nabla x \tilde f \|^2\right]\leq T^{-1/2}(\Delta_0 + L(V + G^2)) $$
\end{theorem}

Finally, we tie the solution of the smoothed problem with that of the original problem (\ref{equ:main_problem}) by using the bound on smooth and regular gradients from \cite{nesterov2017random}.

\begin{theorem}
	With $f_v \in C^{1,1}$, then 
	\begin{equation}
	K_\varepsilon \leq \mathcal{O} \left(\varepsilon^{-2}\right)
	\end{equation}
\end{theorem}

\begin{proof}
	\begin{equation}
	\begin{split}
	\frac{1}{T} \sum_{i = 1}^T \E \left[\|\nabla \tilde f_i\|^2 \right] &\leq  \frac{2}{T} \sum_{i = 1}^T \E\left[\|\nabla f - \nabla \tilde f\|^2\right] + \sum_{i = 1}^T\E\left[\|\nabla \tilde f\|^2\right]\\
	& \leq \frac{2}{T} \sum_{i = 1}^T \left(\frac{\mu}{2} \left(n+3\right)^{3/2}\right)^2 + 2T^{-1/2}C_2\\
	& \leq \frac{\mu^2(n+3)^3}{2}  + 2T^{-1/2}C_2\\
	\end{split}
	\end{equation}
	By selecting $\mu = T^{-1/4}$, we get 
	\begin{equation}
	\frac{1}{T} \sum_{i = 1}^T \E \left[\|\nabla \tilde f_i\|^2 \right] \leq  T^{-1/2}\left(\frac{(n+3)^3}{2} + 2C_2\right)
	\end{equation}
	So that 
	\begin{equation}
	K_\varepsilon \leq \mathcal{O}\left(\varepsilon^{-2}\right)
	\end{equation}
	
\end{proof}
\section{Problem Formulation (Alternate)}
Let $\mathcal{X}$ and $\mathcal{Y}$ be closed and compact subsets of $\mathbb{R}^n$ and $\mathbb{R}^m$ respectively. Define functions $f : \mathcal{Y} \to \mathbb{R}$ and $\phi: \mathcal{X} \to \mathcal{Y}$ such that the problem of interest is to minimize $f$ over the class of functions $\phi \in \Phi$
%
\begin{equation}
\min_{\phi \in \Phi} \mathbb{E}_\mathcal{X}f(\phi(x)).
\end{equation}
%
Instead of minimizing over an arbitrary function class, consider parametrizing $\phi$ by some $\theta \in \Theta$ so that the problem becomes 
%
\begin{equation}
\min_{\theta \in \Theta} \mathbb{E}_\mathcal{X}f(\phi(x,\theta)).
\end{equation}
%
We can solve this problem using stochastic gradient descent (SGD) with stepsize $\eta > 0$, so that the update of the parameter is governed by 
%
\begin{equation}
\theta' = \theta + \eta \nabla_\theta \mathbb{E}_\mathcal{X}f(\phi(x,\theta)).
\end{equation}
% 
By assumption \ref{asm:DCT_cond}, we can move the gradient inside the expectation. Using the chain rule, we have 
%
\begin{equation}\label{equ:our_pol_grad}
\nabla_\theta \mathbb{E}_\mathcal{X} f(\phi(x,\theta)) = \mathbb{E}_\mathcal{X} \left[ \nabla_\theta \phi(x,\theta) \nabla_\phi f(\phi(x,\theta))\right]
\end{equation}
% 
In particular, we are interested in the problem where only zeroth order of the function is available. Zeroth order methods work on a smoothed surrogate function $\tilde f : \mathcal{Y} \to \mathbb{R}$ where the surrogate is defined by smoothing parameter $\mu > 0$
%
\begin{equation}
\tilde f(y) := \mathbb{E}_{u \sim \mathcal{N}(0,I_m)} f(y + \mu u).
\end{equation}
%
By \cite{nesterov2017random}, we know 
\begin{equation}
\sup_{y \in \mathcal{Y}} |\tilde f(y) - f(y) | \leq \mu L \sqrt{N},
\end{equation}
%
and 
\begin{equation}
\nabla \tilde f(y) \equiv \mathbb{E} \left\{\frac{f(y + \mu u) - f(y)}{\mu} u \right\}.
\end{equation}
%
Therefore, to solve 



